LIQUID: A Framework for List Question Answering Dataset Generation

Question answering (QA) models often rely on large-scale training datasets, which necessitates the development of a data generation framework to reduce the cost of manual annotations. Although several recent studies have aimed to generate synthetic questions with single-span answers, no study has been conducted on the creation of list questions with multiple, non-contiguous spans as answers. To address this gap, we propose LIQUID, an automated framework for generating list QA datasets from unlabeled corpora. We first convert a passage from Wikipedia or PubMed into a summary and extract named entities from the summarized text as candidate answers. This allows us to select answers that are semantically correlated in context and is, therefore, suitable for constructing list questions. We then create questions using an off-the-shelf question generator with the extracted entities and original passage. Finally, iterative filtering and answer expansion are performed to ensure the accuracy and completeness of the answers. Using our synthetic data, we significantly improve the performance of the previous best list QA models by exact-match F1 scores of 5.0 on MultiSpanQA, 1.9 on Quoref, and 2.8 averaged across three BioASQ benchmarks.

==> sections/00_preliminaries.tex <==


\section{Preliminaries}
\label{sec:related_work}

This section describe how prior works create factoid questions and why we cannot adopt their methods to list QA data generation.

\paragraph{Answer Extraction}

\paragraph{Question Generation}
Question generation (QG) is the task of generate questions from a passage or document.
% 현존하는 
% factoid question은 수가 많은 반면 list는 그렇지 않음.

While previous works model the probability as $f_\text{QG}(q|[a;c])$, we model $f_\text{QG}(q|[\mathbf{A};c])$, where $\mathbf{A} = \{a_1,\dots,a_T\}$ is the set of answers.

There are public datasets consisting of factoid questions that have a single short answer~\cite{rajpurkar-etal-2016-squad,trischler-etal-2017-newsqa,joshi-etal-2017-triviaqa,kwiatkowski2019natural}

\paragraph{Filtering}



==> sections/5_related_work.tex <==

\section{Related Work}

\subsection{List Question Answering Datasets}

Extractive QA does not limit the number of answer spans and includes questions that require exact one span, no answer span, and multiple spans.
Although recent studies are building large extractive QA datasets~\cite{rajpurkar-etal-2016-squad,trischler-etal-2017-newsqa,joshi-etal-2017-triviaqa,rajpurkar-etal-2018-know,yang-etal-2018-hotpotqa,kwiatkowski2019natural}, they largely consist of single-span factoid or unanswerable questions and have only few list questions.
The \bioasq~challenge~\cite{tsatsaronis2015overview} continues its efforts to hand-label new list questions in the biomedical QA research.
Recently, \citet{li2022multispanqa}~proposed the \multispanqa~dataset for training and evaluating list QA models.
Unfortunately, the training data is still limited to achieve satisfactory list QA performance.
To alleviate the data scarcity problem, this study presented a list QA dataset generation framework for the first time.


\subsection{QA Dataset Generation}

\citet{alberti-etal-2019-synthetic} first proposed a three-step framework (i.e., answer extraction, question generation, and roundtrip filtering) frequently used in studies on QA data generation and showed synthetic data could enhance QA performance.
Recent advances in large-scale sequence-to-sequence models~\cite{radford2019language,lewis-etal-2020-bart,raffel2020exploring} have further improved the quality of generated datasets, making them more useful in QA~\cite{puri-etal-2020-training,shakeri-etal-2020-end,lewis-etal-2021-paq}.
However, their models cannot be applicable to list QA generation due to its unique characteristics and challenges, as mentioned in \Cref{sec:intro}.
On the other hand, our framework, designed for list QA, has shown to be effective on different benchmarks.


==> sections/C_leaderboard.tex <==

\section{Leaderboard Evaluation}
\label{appendix:leaderboard}

\input{tables/leaderboard}

Our RoBERTa-base model was first submitted on August 9, 2022. 
To determine if our synthetic data improves larger QA models, we trained a sequence labeling model based on RoBERTa-large and evaluated it on the MultiSpanQA leaderboard. 
\Cref{tab:leaderboard}~presents that we improved the performance of the QA model by an F1 score of 5.0.
In addition, our best model (ensemble) achieved a new SOTA performance on October 14th.



==> tables/case_study.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{adjustbox}{max width = 0.99\columnwidth}

\begin{tabular}{ll}
\toprule
\textbf{Text Source} & \textbf{Example}  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Original text\end{tabular} & \begin{tabular}[c]{@{}l@{}}Q: Which governing bodies have veto power? \\
Sen.: The European Parliament and \\the Council of the European Union have \\powers of amendment and veto during \\the legislative process.\end{tabular} \\
\midrule
Summary & \begin{tabular}[c]{@{}l@{}}Q: Which governing bodies have veto power? \\
Sen.: The European Parliament and \\the Council of the European Union have \\powers of amendment and veto during \\the legislative process.\end{tabular} \\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{
adsf
}
\label{tab:case_study}
\end{table}

==> tables/hyperparams_inference.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{llc}
\toprule
\textbf{Model} & \textbf{Hyperparameter} & \textbf{Value} \\
\midrule
Summarization & Maximum output length & 128 \\
\midrule
QG Model & Maximum output length & 128  \\
\midrule
QA Model & Maximum input length & \\
 & Threshold & \\
\bottomrule
\end{tabular}
\end{table}

==> tables/leaderboard.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\begin{tabular}{llcccc}
\toprule
\multirow{2}{*}{\textbf{Team}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Validation}} & \multicolumn{2}{c}{\textbf{Test}} \\
 && \textbf{Exact F1 (P/R)} & \multicolumn{1}{l}{\textbf{Partial F1 (P/R)}} & \textbf{Exact F1 (P/R)} & \multicolumn{1}{l}{\textbf{Partial F1 (P/R)}} \\
\midrule
\citet{li2022multispanqa} & BERT-base Single-span  & - & - & 14.4 (16.2/13.0) & 67.6 (60.3/76.8) \\
& BERT-base Tagger & - & - & 56.5 (52.5/61.1) & 75.2 (75.9/74.5) \\
& BERT-base Tagger (multi-task) & - & - & 59.3 (58.1/60.5) & 76.3 (79.6/73.2) \\
\midrule
Illuin Technology & RoBERTa-large Tagger & - & - & 69.2 (68.1/70.3) & 83.9 (85.6/82.2) \\
\midrule
Anonymous & Qualifier (BERT-base) & - & - & 64.9 (63.6/66.2) & 78.8 (78.0/79.6) \\
& Qualifier (RoBERTa-large) & - & - & 72.8 (72.4/{73.1}) & \textbf{85.4} (85.3/85.5) \\
\midrule
Our team & RoBERTa-base Tagger & 67.5 (64.5/70.9) & 82.6 (82.4/82.8) & 62.9 (63.0/62.9) & 78.0 (82.5/73.9) \\
& \quad + LIQUID & 73.0 (72.0/74.0) & 84.4 (85.5/83.3) & 67.4 (65.7/69.2) & 81.2 (80.9/81.5) \\
& RoBERTa-large Tagger & 72.8 (70.0/75.7) & 87.4 (87.3/87.6) & 66.4 (62.3/71.2) & 82.6 (82.1/83.0) \\
& \quad+ LIQUID & 76.2 (77.9/74.6) & 85.9 (89.0/83.0) & 71.4 ({75.0}/68.2) & 80.9 (85.3/77.0) \\
& \quad+ LIQUID (Ensemble) & \textbf{77.8} ({78.3}/{77.2}) & \textbf{87.4} (89.3/85.7) & \textbf{73.1} (74.3/72.0) & 83.4 (85.6/81.3) \\
\bottomrule
\end{tabular}
\caption{leaderboard results}
\label{tab:leaderboard}
\vspace{-3mm}
\end{table*}

==> tables/model_config.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\begin{tabular}{lllll}
\toprule
\textbf{Type} & \textbf{Summarizaiton} & \textbf{Answer Extraction} & \textbf{Question Generation} & \textbf{Iterative Filtering} \\
\midrule
\multicolumn{5}{l}{\textit{General domain}} \\
\midrule
Backbone model & BART & \multirow{2}{*}{SpaCy} & T5 & RoBERTa \\
Training data & CNN/Daily Mail &  & SQuAD & SQuAD \\
\midrule
\multicolumn{5}{l}{\textit{Biomedical domain}} \\
\midrule
Backbone model & BioBART & \multirow{2}{*}{BERN 2} & T5 & PubMedBERT \\
Training data &  &  & \squad $\rightarrow$ \bioasq~6b & \squad $\rightarrow$ \bioasq~6b \\
\bottomrule
\end{tabular}
\caption{config}
\label{tab:model_config}
\end{table*}

==> tables/transfer.tex <==

\begin{table}[]
\centering
\footnotesize
\begin{adjustbox}{max width = 0.99\columnwidth}

\begin{tabular}{lcccccc}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Fine-\\tuning\end{tabular}}} & \multicolumn{3}{c}{\textbf{\multispanqa}} & \multicolumn{3}{c}{\textbf{\bioasq~9b}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \textbf{List} & \textbf{Factoid} & \textbf{Both} & \textbf{List} & \textbf{Factoid} & \textbf{Both} \\
\midrule
List & xx.x & xx.x & xx.x & 61.8 & 71.9 & xx.x \\
Factoid & xx.x & xx.x & xx.x & 49.0 & 80.2 & xx.x  \\
Both &  & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{asdf}
\label{tab:transfer}
\end{table}
